One Explanation Does Not Fit XIL

Current machine learning models produce outstanding results in many areas but, at the same time, suffer from shortcut learning and spurious correlations. To address such flaws, the explanatory interactive machine learning (XIL) framework has been proposed to revise a model by employing user feedback on a model's explanation. This work sheds light on the explanations used within this framework. In particular, we investigate simultaneous model revision through multiple explanation methods. To this end, we identified that \textit{one explanation does not fit XIL} and propose considering multiple ones when revising models via XIL.

==> old_code.tex <==
\begin{table}[]
    \centering
    \def\arraystretch{1}\tabcolsep=2.pt
    \begin{tabular}{c|c|ccccccc}
        & w/o decoy & Vanilla & RRR & RRR-G & HINT & CDEP & RRR+RRR-G & RRR-G+HINT \\ \hline
        train & 1& 1& 1& 1& 1& 1& 1& 1 \\
        test  & 1& 1& 1& 1& 1& 1& 1& 1
        %train & $99.8$ & $98.8$ \\ \hline
        %test & Vanilla & $99.9$ & $78.9$ \\ \hline
        %RRR & $99.9$ & $98.8$ \\
        %RRR-G & $99.7$ & $97.4$ \\
        %RBR & $\mathbf{100.0}$ & $\mathbf{99.1}$  \\
        %CDEP & $99.3$ & $97.1$&  \\
        % & 
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\begin{table}[t]
    \centering
    \def\arraystretch{1}\tabcolsep=3.pt
    \begin{tabular}{cc|c}
        % \multicolumn{1}{c}{} & \multicolumn{2}{c}{DecoyMNIST} \\
        XIL & train & test \\ \hline 
        w/o decoy & $99.8$ & $98.8$ \\ \hline
        Vanilla & $99.9$ & $78.9$ \\ \hline
        RRR & $99.9$ & $98.8$ \\
        RRR-G & $99.7$ & $97.4$ \\
        RBR & $\mathbf{100.0}$ & $\mathbf{99.1}$  \\
        CDEP & $99.3$ & $97.1$
        % HINT & $97.6$ & $96.6$ \\
        % CE & $99.9$ & $98.9$ \\ 
    \end{tabular}
    \quad
    % \begin{tabular}{c|c}
    %     \multicolumn{2}{c}{DecoyFMNIST} \\
    %     train & test \\ \hline
    %     $99.5$ & $58.3$\\ \hline
    %     $98.7$ & $\mathbf{89.4}$ \\ 
    %     $90.2$ & $78.6$ \\ 
    %     $96.6$ & $87.6$ \\ 
    %     $89.8$ & $76.7$  \\ 
    %     $99.0$ & $58.2$ \\ 
    %     $\mathbf{99.1}$ & $87.7$ \\
    % \end{tabular}
    % \quad
%     \caption{Mean accuracy scores of single XIL methods [\%]. First row shows the Vanilla model (no XIL) gets fooled, indicated by low test accuracy. Except HINT on FMNIST, all methods recover test accuracy. Best values are \textbf{bold}; cross-validated on 5 runs}
%     \label{tab:exp_performance}
% \end{table}
% \begin{table}[H]
%     \centering
%     \def\arraystretch{1}\tabcolsep=3.pt
    \begin{tabular}{cc|c}
        % \multicolumn{1}{c}{} & \multicolumn{2}{c}{DecoyMNIST} \\
        XIL & train & test \\ \hline 
        RRR + RRR-G + RBR & $98.8$ & $98.3$ \\
        RRR + CDEP & $99.3$ & $98.5$ \\
        RRR + RBR & $99.9$ & $\mathbf{98.9}$ \\
        RBR + CDEP & $99.2$ & $98.6$ \\
        RRR-G + CDEP & $98$ & $96.6$ \\ 
        % \hline
        % RRR-G + HINT & $93.2$ & $94.6$ \\
        % CDEP + HINT & $97.7$ & $\mathbf{97.4}$ \\
        % RRR + HINT & $93.4$ & $94.4$ \\
        % RBR + HINT & $95$ & $95.4$ \\ \hline
        % RRR + CE & $99.9$ & $98.8$ \\
        % RBR + CE & $100$ & $\mathbf{99.1}$ \\
        % RRR-G + CE & $97.7$ & $96.7$ \\
        % CDEP + CE & $99.7$ & $98.4$ \\
        % HINT + CE & $98.4$ & $97.4$ \\
    \end{tabular}
    % \quad
    % \begin{tabular}{c|c}
    %     \multicolumn{2}{c}{DecoyFMNIST} \\
    %     train & test \\ \hline
    %     $92$ & $88.4$ \\
    %     $98.2$ & $88.4$ \\
    %     $98.5$ & $\mathbf{89.5}$ \\
    %     $87$ & $87$ \\
    %     $86.3$ & $81.2$ \\ \hline
    %     $89.6$ & $77.3$ \\
    %     $89.8$ & $75.9$ \\
    %     $93.4$ & $\mathbf{89.4}$ \\
    %     $94.5$ & $84.9$ \\ \hline
    %     $99.2$ & $\mathbf{89.3}$ \\
    %     $94$ & $85.2$ \\
    %     $94.6$ & $86.4$ \\
    %     $94.1$ & $86.1$ \\
    %     $93$ & $87.3$ \\
    % \end{tabular}
    % \quad
    \caption{XIL Accuracy [\%] on DecoyMNIST. The Vanilla model without XIL gets fooled. Single and combinations of XIL methods help achieve same performance as without decoy.}
    % Mean accuracy scores [\%] of XIL methods combination. The first 5 rows show combinations of XIL methods with different internally-used explainer. The next 4 rows shows combinations of XIL methods that use penalty and reward strategy. The last 5 rows shows combinations of XIL methods that adopt loss augmentation and dataset augmentation. Best values of each kind of combination are \textbf{bold}; cross-validated on 5 runs}
    \label{tab:accuracy}
\end{table}


\begin{table*}[h!]
    \centering
    \def\arraystretch{1}\tabcolsep=2.pt
    \begin{tabular}{c|c|c|c|c}
        %\multicolumn{1}{c}{} & \multicolumn{4}{c}{DecoyMNIST} \\
        Explainer(s) & RRR-G+HINT & CDEP+HINT & RRR+HINT & RBR+HINT \\ \hline 
        
        IG & $1.0 \pm0.5$ & $0.3\pm0.1$ & $\mathbf{0.0}\pm0.0$ & $0.8\pm0.4$\\
        
        GradCAM & $\mathbf{3.0}\pm0.3$ & $3.2\pm0.2$ & $5.3\pm1.0$ & $3.9\pm1.0$\\
        
        LIME & $30.1\pm5.3$ & $31.0\pm0.5$ & $27.4\pm1.2$ & $\mathbf{27.3}\pm0.9$\\ 
        
        % Saliency & $0.2\pm 0.11$ & $\mathbf{0.0}\pm0.0$ & $\mathbf{0.0}\pm0.0$ & $0.2\pm0.0$\\ 
        
        IxG & $9.9\pm1.7$ & $5.9 \pm1.5$ & $\mathbf{0.9}\pm0.4$ & $8.8\pm1.3$ \\
        
        DeepLift & $9.6 \pm2.2$ & $5.7\pm1.4$& $\mathbf{0.8}\pm0.4$ & $8.4\pm1.1$\\ 
        
        % LRP & $9.9\pm1.7$ & $5.9 \pm1.5$ & $\mathbf{0.9}\pm0.4$ & $8.8\pm1.3$ \\
        
        GBP & $5.7\pm3.6$ & $5.3 \pm1.4$ & $\mathbf{0.0}\pm0.0$ & $3.5\pm2.2$ \\
        
        IntGrad & $8.5\pm0.8$ & $5.6\pm2.8$ & $\mathbf{1.4}\pm1.0$ & $8.5\pm1.4$ \\
    \end{tabular}
    %\quad
    \caption{test}
    % Mean \wrmetric scores of combinations of XIL methods that adopt penalty and reward strategy on MNIST dataset[\%]. Lower is better; best values for each explainer are \textbf{bold}; cross-validated on 5 runs with standard deviation.}
    \label{tab:exp_wr_mix_comb_2_mnist}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Result tables from the thesis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[H]
    \centering
    \def\arraystretch{1}\tabcolsep=3.pt
    \begin{tabular}{c|c|c}
        \multicolumn{1}{c}{} & \multicolumn{2}{c}{DecoyMNIST} \\
        XIL & train & test \\ \hline 
        RRR + RBR + RRR-G & $98.8$ & $98.3$ \\
        RRR + CDEP & $99.3$ & $98.5$ \\
        RRR + RBR & $99.9$ & $\mathbf{98.9}$ \\
        RBR + CDEP & $99.2$ & $98.6$ \\
        RRR-G + CDEP & $98$ & $96.6$ \\ \hline
        RRR-G + HINT & $93.2$ & $94.6$ \\
        CDEP + HINT & $97.7$ & $\mathbf{97.4}$ \\
        RRR + HINT & $93.4$ & $94.4$ \\
        RBR + HINT & $95$ & $95.4$ \\ \hline
        RRR + CE & $99.9$ & $98.8$ \\
        RBR + CE & $100$ & $\mathbf{99.1}$ \\
        RRR-G + CE & $97.7$ & $96.7$ \\
        CDEP + CE & $99.7$ & $98.4$ \\
        HINT + CE & $98.4$ & $97.4$ \\
         
    \end{tabular}
    \quad
    \begin{tabular}{c|c}
        \multicolumn{2}{c}{DecoyFMNIST} \\
        train & test \\ \hline
        $92$ & $88.4$ \\
        $98.2$ & $88.4$ \\
        $98.5$ & $\mathbf{89.5}$ \\
        $87$ & $87$ \\
        $86.3$ & $81.2$ \\ \hline
        $89.6$ & $77.3$ \\
        $89.8$ & $75.9$ \\
        $93.4$ & $\mathbf{89.4}$ \\
        $94.5$ & $84.9$ \\ \hline
        $99.2$ & $\mathbf{89.3}$ \\
        $94$ & $85.2$ \\
        $94.6$ & $86.4$ \\
        $94.1$ & $86.1$ \\
        $93$ & $87.3$ \\
    \end{tabular}
    \quad
    \caption{Mean accuracy scores [\%] of XIL methods combination. The first 5 rows show combinations of XIL methods with different internally-used explainer. The next 4 rows shows combinations of XIL methods that use penalty and reward strategy. The last 5 rows shows combinations of XIL methods that adopt loss augmentation and dataset augmentation. Best values of each kind of combination are \textbf{bold}; cross-validated on 5 runs}
    \label{tab:accuracy2}
\end{table}
